Mechanism Design for Cumulative Prospect Theoretic Agents: A General Framework and the Revelation Principle

This paper initiates a discussion of mechanism design when the participating agents exhibit preferences that deviate from expected utility theory (EUT). In particular, we consider mechanism design for systems where the agents are modeled as having cumulative prospect theory (CPT) preferences, which is a generalization of EUT preferences. We point out some of the key modifications needed in the theory of mechanism design that arise from agents having CPT preferences and some of the shortcomings of the classical mechanism design framework. In particular, we show that the revelation principle, which has traditionally played a fundamental role in mechanism design, does not continue to hold under CPT. We develop an appropriate framework that we call mediated mechanism design which allows us to recover the revelation principle for CPT agents. We conclude with some interesting directions for future work.

==> tex/ex_valUF_x.tex <==
%!TEX root = ../main.tex

\begin{figure}
\centering
\begin{tikzpicture}[scale = 1]
    \begin{axis}[
    	xmin = 0,
    	xmax = 1,
    	ymin = -75,
    	ymax = -65,
        xlabel=$x$,
        ylabel=$E(x)$,
        every axis plot/.append style={ultra thick},
        %legend style={ at={(0.4,0.9)}, anchor=north east, align=left, draw=white!15!black}
        ]
\addplot []
  table[row sep=crcr]{%
	0   -68.7500\\
    0.25   -73.1250\\
    0.5   -66.25\\
    1   -71.2500\\
};
%\addlegendentry{Gains}


% \addplot[smooth, loosely dotted] plot coordinates {
%         (0,0)
%         (1, 1)
% };
%\addlegendentry{Bob}

\end{axis}
\end{tikzpicture}%
\caption{Plot of expression $E(x)$ in Claim~\ref{cl: ex_valuUF}.}
\label{fig: ex_valUF}
\end{figure}
